Understanding Politics via Contextualized Discourse Processing

Politicians often have underlying agendas when reacting to events. Arguments in contexts of various events reflect a fairly consistent set of agendas for a given entity. In spite of recent advances in Pretrained Language Models (PLMs), those text representations are not designed to capture such nuanced patterns. In this paper, we propose a Compositional Reader model consisting of encoder and composer modules, that attempts to capture and leverage such information to generate more effective representations for entities, issues, and events. These representations are contextualized by tweets, press releases, issues, news articles, and participating entities. Our model can process several documents at once and generate composed representations for multiple entities over several issues or events. Via qualitative and quantitative empirical analysis, we show that these representations are meaningful and effective.

==> reproducibility.tex <==
We use seeds (set to $4056$ for both tasks) for both random example generation and training neural networks. For fine-tuning layers of learning tasks we initialize the models using Xavier uniform \citep{xavier-init-2010} initialization with gain=$1.0$. We optimize the parameters using Stochastic Gradient Descent with an initial learning rate=$0.0075$ and momentum=$0.4$. We used $4$ Nvidia GeForce GTX $1080$ Ti GPUs with $12$ GB memory and linux servers with $64$ GB RAM for our experiments. CPU RAM and GPU memory are the main bottlenecks for training the model. It takes $80$ hours to train authorship prediction for $5$ epochs and $14$ hours to train referenced entity prediction task for the same. Generating test results for both tasks together takes $3$ hours. We use a batch size of $1$ for both training and evaluation. For NRA Grade Prediction task we use $5$ random seeds: \{$5, 7, 11, 13, 17$\} and report mean and standard deviation. The encoder-composer architecture is made up of $8.26$M parameters, encoder consisting of $3.54M$ and composer $4.72M$. Due to long training time, the only hyperparameter we experimented with is the graph size. We retained as many nodes as possible without exceeding GPU memory ($500$ nodes). Our code and processed data are released\footnote{\url{https://github.com/pujari-rajkumar/compositional_learner}}.\\
\indent We divide the $3,640$ queries into $151$ batches of $24$ queries each ($3$ politicians $\times$ $8$ issues) and $1$ batch of $16$ queries ($2$ politicians $\times$ $8$ issues). Train, val and test data examples are generated for each query batch.  For Authorship Prediction and Referenced Entity Prediction tasks, Compositional Reader model is trained on one batch for $5$ epochs, the best parameters are chosen according to the validation performance of that batch and we proceed to training on future batches. Politicians are ordered randomly when generating queries.

\subsection{Data Collection}
We collected data from $5$ sources: Wikipedia, Twitter, \href{https://www.ontheissues.org}{ontheissues.org}, \href{https://www.allsides.com}{allsides.com} and ProPublica Congress API. We scraped articles from Wikipedia related to all the politicians in focus. We collected tweets from \href{https://github.com/alexlitel/congresstweets}{Congress Tweets} and \citet{trump-tweets-2019}. We used a set of hand build gold hashtags to separate them by issues. They are shown at the end of this document. We collected all news articles related to the $8$ issues in focus from \href{https://www.allsides.com}{allsides.com}. We collected press releases from Propublica API using key word search. We use issue names as keywords.

    

